17 and 24 GHz observations of southern pulsars

We present observations of PSRs J0437-4715, J0738-4042, J0835-4510, J0908-4913, J1048-5832, J1622-4950, J1644-4559, J1721-3532 and J1740-3015 at 17 GHz using the Parkes radio telescope. All 9 were detected at 17 GHz, additionally, we detected PSR J0835-4510 and J1622-4950 at 24 GHz. Polarisation profiles of each pulsar and the variation with frequency are discussed. In general, we find that the highly polarised edge components of young pulsars continue to dominate their profiles at 17 GHz. Older pulsars (>10^5 years) appear to be almost completely depolarised. Our detection of PSR J0437-4715 is the highest frequency observation of a millisecond pulsar to date, and implies a luminosity at 17 GHz of 14 {\mu}Jy kpc^2, and a mean spectral index of 2.2. We find that the spectral index of the magnetar PSR J1622-4950 is flat between 1.4 and 24 GHz, similar to the other known radio magnetars XTE J1810-197 and 1E 1547.0-5408. The profile is similar to that at 3.1 GHz, and is highly linearly polarised. Analysis of the frequency evolution of the profile of PSR J0835-4510 show that the profile is made of four components that vary with frequency only in their amplitude. The width and separation of the components remains fixed and the spectral index of each component can be determined independently.

==> makefigs <==
#!/bin/bash

for i in *_*.eps; do 
n=`basename $i .ps`
echo "\begin{figure}"
echo "\includegraphics[height=8cm]{$i}"
echo "\caption{"
echo "\label{$n}"
echo "}"
echo "\end{figure}"
done




